GNNAdvisor: An Adaptive and Efficient Runtime System for GNN Acceleration on GPUs

As the emerging trend of graph-based deep learning, Graph Neural Networks (GNNs) excel for their capability to generate high-quality node feature vectors (embeddings). However, the existing one-size-fits-all GNN implementations are insufficient to catch up with the evolving GNN architectures, the ever-increasing graph sizes, and the diverse node embedding dimensionalities. To this end, we propose \textbf{GNNAdvisor}, an adaptive and efficient runtime system to accelerate various GNN workloads on GPU platforms. First, GNNAdvisor explores and identifies several performance-relevant features from both the GNN model and the input graph, and uses them as a new driving force for GNN acceleration. Second, GNNAdvisor implements a novel and highly-efficient 2D workload management, tailored for GNN computation to improve GPU utilization and performance under different application settings. Third, GNNAdvisor capitalizes on the GPU memory hierarchy for acceleration by gracefully coordinating the execution of GNNs according to the characteristics of the GPU memory structure and GNN workloads. Furthermore, to enable automatic runtime optimization, GNNAdvisor incorporates a lightweight analytical model for an effective design parameter search. Extensive experiments show that GNNAdvisor outperforms the state-of-the-art GNN computing frameworks, such as Deep Graph Library ($3.02\times$ faster on average) and NeuGraph (up to $4.10\times$ faster), on mainstream GNN architectures across various datasets.

==> 04_new_GPU_workload_management.tex <==
\section{2D Neighbor-Dimension Workload} 
\label{sect: Group-based Workload Management}
\begin{figure*} [h] \small
    \centering
    \includegraphics[width=\textwidth]{imgs/2D-neighbor-dim.pdf}
    \caption{2D Dimension Partitioning.}
    \label{fig: 2D Dimension Partitioning}
\end{figure*}
\Mname~incorporates a 2D neighbor-dimension workload management tailored for vector-based GNN computing. It includes a 2D neighbor-dimension workload partitioning and a lightweight multi-level synchronization.
% its GNN-tailored group-based workload management with four techniques: 
% \textit{group-based partitioning}, \textit{leader-node scheme}, \textit{block-based mapping}, and \textit{dimension-based sharing}.
%\Mname~features its group-based workload management by taking node degree and embedding into consideration. It consists of four major techniques: group-based partitioning, leader-node scheme, block-based mapping, and dimension-based sharing.
% optimize its execution by mapping workloads to GPU based on its hardware-level properties.

% \subsection{Group-based Partitioning}
\subsection{2D Neighbor-Dimension Partitioning}
\label{sect: Group-based Partitioning}
Unlike the traditional graph processing that each node is only represented by a scalar value, GNN computing highlights its speciality with each node represented by a feature vector. The most basic workload unit is the element-wise vector addition between a node and one of its neighbors, which usually takes $O(d)$ time complexity ($d$ is the vector dimension). 

To better analyze the GNN workload, we first propose a novel GNN workload spatial abstraction with three different dimensions: \textit{node}, \textit{neighbor}, and \textit{dimension (dim)}, each of which is orthogonal to the other two. As shown in Figure~\ref{fig: 2D Dimension Partitioning}, each long rectangular box represents the workload from one neighbor node, and neighbors workload of different nodes are denoted in different colors. \todo{From this abstraction, we can summarize two challenges: 1) workloads across different nodes are different from each other, leading to imbalanced workload according the power-law degree distribution of most real-word graphs; 2) workloads of the same node would vary with the vector dimension, since GNN computation usually consists of multiple layers with different hidden dimensions.}
% One key challenge here is how could we split the workload to benefit single-thread efficiency and multi-thread parallelism. This requires assigning appropriate loads to each thread and organizing thread in an efficient and collaborative way.
To tackle these challenges, we propose a 2D neighbor-dimension partitioning for workload balancing and computation parallelization. It consists of two major steps.

\paragraph{Coarse-grained Neighbor Split:} It is the first steps of our 2D neighbor-dimension partitioning, which splits the workloads along the neighbor dimension of each node to resolve the inter-node workload imbalance. Take the node c in Figure~\ref{fig: 2D Dimension Partitioning} for illustration, neighbor partition divides the original workloads of node c into three equal-sized neighbor-parts: \textit{np-1}, \textit{np-2}, and \textit{np-3} (denoted by three different colors). Note that this step is an initial coarse-grained workload partitioning, and its output will be used for a more fine-grained workload partitioning along the dimension axis.
% neighbor split offer better workload granularity.

\paragraph{Fine-grained Dimension Split:} It slices the workloads along the dimension axis for parallelization after the coarse-grained neighbor split. The dimension of each vector is further divided in to equal-sized dimension-pieces. As shown in Figure~\ref{fig: 2D Dimension Partitioning}, the aggregation workload of \textit{np-1} for node $a$ is breakdown into three different dimension-pieces: \textit{dp-1}, \textit{dp-2}, and \textit{dp-3}, denoted by the boxes with the same color but different color depths. There are two types of breakdown, the first one is the sequential breakdown (Figure~\ref{fig: 2D Dimension Partitioning}\todo{add subfig}), and the second is the cyclic split (Figure~\ref{fig: 2D Dimension Partitioning}\todo{subfig}) for benefiting memory coalescing in GPUs.

\paragraph{Hyper-Parameter Selection:} It basically determines the value of size of the neighbor-parts and dimension-piece. We use the node degree and node embedding vector size to guide our selection. We select the node average degree of a graph as the size of the neighbor-part in general to balance workload granularity and ease of fine-grained dimension split. To select the size of dimension piece, we use the following formula,
\begin{equation} \small
    dp\_size =  \frac{shared\_mem}{avg\_degree\times Dtype\times max\_threadPerBlock}
\end{equation}
where Dtype is 4 bytes for single-precision floating-point for most GPU computations, $max\_threadPerBlock$ is 1024 in general for modern GPUs, $shared\_mem$ is a GPU-specific hardware parameter at KB level (<100 KB). 

After the above 2D neighbor-dimension splits with appropriated hyper-parameters, we build the basic \textit{workload unit} (consists of boxes with the same color and color depths) of a node that can be indexed by its unique neighbor-part and dimension-piece index. We assign one such workload unit to a GPU thread for execution.

% dimension-axis cyclic distribution, we also spot the memory access pattern as a key factor to bring even better performance, since threads with continuous IDs will access to a consecutive part of memory, thus facilitating the memory coalescing on GPUs. To this end, as shown in Figure~\ref{fig: 2D Dimension Partitioning}\subfig{b}, we adjust the threads and their workload mapping, where adjacent threads would operate on the dimension close to each other side by side.
% The benefits of applying the group-based aggregation are three-fold: 1) compared with the more coarse-grained node-centric aggregation (Figure~\ref{fig: Group-based aggregration}\subfig{b}), which distributes workloads by nodes, group-based partitioning can largely mitigate the inter-thread imbalance by dividing workloads into groups that are set to be equal in size; 2) compared with the more fine-grained edge-centric aggregation (Figure~\ref{fig: Group-based aggregration}\subfig{b}), which is seemingly high-performance by using more threads for massive parallelism, the group-based solution can avoid the overheads of managing excessive threads that might hurt the performance in many ways, such as resource contentions, and synchronizations. 
% To this end, our 2D neighbor-dimension partitioning is designed to handle GNN-specific workloads. As shown in Figure~\ref{fig: workload}
% To this end, we propose a novel 2D neighbor-dimension partitioning, which resolve the workload imbalance from two cardinals: the neighbor and the dimension. workload balancing along neighbors.
% global view and local view of the design 
% As shown in Figure~\ref{}, the neighbors of each node along with its dimension could be consider as a 2D mesh. We basically have two types of splits: x-split and y-split, which are designed for workload balancing and parallelism on neighbors and dimension. Figure~\ref{} shows an example of initial partitioning on neighbors, which partitioning the node neighbors into different parts based on a pre-determined partitioning size K, therefore we can have n different partitioning on the neighbor-axis. 
% \subsection{Dimension-axis Partitioning}
% GNN distinguishes itself from traditional graph algorithms in its computation on high-dimension node embeddings. To tackle this challenge efficiently, we further offload the group-based workloads from a single thread to a group of threads to improve the aggregation performance through dimension-based workload sharing. As shown in Figure~\ref{fig: Dimension-based Workload Sharing.}\subfig{a}, the original group-based workloads are distributed to three different working threads for workload sharing. And each thread manages a part of (around 1/3) workload during the node aggregation. There are two benefits of applying this strategy. First, it could effectively execute the node aggregation on a diverse range of the node embedding dimension and the GNNs' hidden dimension, since the group-based workload can be shared by multiple threads instead of single thread. 
% % Second, it would facilitate more efficient data access, such as memory coalescing, to improve memory performance. 
% Second, it introduces another performance-related parameter -- the number of working threads along the data dimension for configurability.
% However,  












% Group-based workload partitioning is a novel workload balance technique tailored for GNNs on GPUs. It breaks down the neighbors of a node into different groups and assigns the aggregation workload of each group to a thread. 
% \todo{Specifically, it takes three things into consideration. First, the node degrees of a graph, which would determinate the size ($\#nodes$) of each group; Second, the workload per thread, which would decide how much workload can be assigned to each thread that could maximize the single-thread efficiency; Third, the total number threads running simultaneously, which would determine the parallelism of GNN computation.} 
% Specifically, it relies on the input-level information -- node degree and node embedding -- to determine the size of each node group and the aggregation workload assigned to each thread. The neighbors of a node are sorted by their ids, and we divided them into different groups based on the selected group-size parameter. And such grouping is a lightweight approach and is done on-the-fly when loading the graph from disk to memory and maintained by a low-cost neighbor-group data structure during the runtime. As shown in Figure~\ref{fig: Group-based aggregration}\subfig{a}, the neighbors of a node are divided into 3 groups with a pre-determined group size of 4. In aggregation, each thread handles the intra-group aggregation workload (\textit{i.e.}, element-wise accumulation of neighbors' embedding vectors). After finishing the intra-group aggregation, an inter-group reduction will gather final results for each node. 
% \todo{how neighbors are organized into different groups}


% To further exploit its performance benefits, we introduce an adjustable parameter -- group size (\textit{i.e.}, $\#node$ in each group), and detail its value selection in Section~\ref{sect: Modeling}. 
% \begin{figure} [h] \small
%     \centering
%     \includegraphics[width=\columnwidth, scale =1.1]{imgs/group-based-aggregration.pdf}
%     \vspace{-15pt}
%     \caption{(a) Group-based Aggregation; (b) Node-centric Aggregation; (c) Edge-centric Aggregation.}
%     % \vspace{-5pt}
%     \label{fig: Group-based aggregration}
% \end{figure}

\subsection{Lightweight Multi-level Synchronization} 
\label{sect: Lightweight Multi-level Synchronization}
While the group-based workload partitioning largely mitigates the workload imbalance and increases the dimension-wise parallelism, the costly thread synchronization would still throttle the overall performance. As shown in Figure~\ref{fig: Lightweight Multi-level Synchronization}\subfig{a}, to accumulate the results of node~\todo{add the node id}, different threads have to competitively update the same part of data. And to guarantee the result correctness, thread-level synchronization (\textit{e.g.}, atomic operations) has to be intensively used, leading to inefficient memory access and performance degradation.
\begin{figure} [h] \small
    \centering
    \includegraphics[width=0.8\columnwidth]{imgs/multi-level-sync.pdf}
    \caption{Lightweight Multi-level Synchronization.\todo{change the figure}}
    \label{fig: Lightweight Multi-level Synchronization}
\end{figure}
To tackle these challenges, \Mname~employs a lightweight multi-level synchronization, which consists of two essential steps: \textit{unit-level sync} and \textit{node-level sync}.
% Each group of neighbor nodes maintain a leader that holds the result of intra-group aggregation temporarily. Since each thread manages aggregation for a neighbor-parts, its execution can be proceeded in an atomic-free manner because of no inter-thread contention. After the intra-group aggregation, a wait-free inter-group reduction will be triggered to gather the final results. Since each thread can start pushing its result to the center node as soon as it finishes its intra-group aggregation. 
% Two dimension sync in different axis to handle the results and synchronization.
\paragraph{Unit-level Sync:} It accumulates the results within a workload unit, and it can be proceeded in an atomic-free manner, since each workload unit is managed by only one GPU thread. In other word, unit-level sync on different workloads can be proceed in parallel with different threads. 
% since each part is managed by a thread, therefore, there is no need for us to output the final result to global memory each time when we do the aggregation. Instead, we can first build a partial result, then,

\paragraph{Node-level Sync:} It collects the final results of each node. For example, node \todo{add ids} will update itself by accumulating the results from different workload units.  This can finished in a wait-free manner, since each thread would use the partial accumulation result to update the node once it has finished its intra-unit accumulation.
% one is wait-free the other is atomic-free, for the dataset with larger dimension ($d>128$), wait-free update would benefits due to more thread to update at the same time, while for lower dimension atomic-free by assigning one thread to update is more beneficial.
Combining unit-level sync and node-level sync, we can reduce 50\% unnecessary atomic operations. 
%at global memory.
% we can follow the similar strategy to reduce the global memory access and part-level header to do synchronization in a non-wait manner. we use the thread from one-part to to synchronization and other part for 
% By combining the above two steps of aggregations at the intra-group and inter-group level, \Mname~aggregation kernel is optimized in its performance by effectively reducing the time and cost for thread-level synchronization (\textit{e.g.}, atomic operations).
% \vspace{-10pt}
% \begin{figure} [h] \small
%     \centering
%     \includegraphics[scale=0.6, height=3cm]{imgs/leader-node-aggregation.pdf}
%     \vspace{-10pt}
%     \caption{Leader-node Aggregation Scheme.}
%     \vspace{-15pt}
%     \label{fig: Leader-node Aggregation.}
% \end{figure}

%\vspace{-5pt}


% \subsection{Dimension-based Sharing} \label{sect: dimension-workload sharing.}
% GNN distinguishes itself from traditional graph algorithms in its computation on high-dimension node embeddings. To tackle this challenge efficiently, we further offload the group-based workloads from a single thread to a group of threads to improve the aggregation performance through dimension-based workload sharing. As shown in Figure~\ref{fig: Dimension-based Workload Sharing.}\subfig{a}, the original group-based workloads are distributed to three different working threads for workload sharing. And each thread manages a part of (around 1/3) workload during the node aggregation. There are two benefits of applying this strategy. First, it could effectively execute the node aggregation on a diverse range of the node embedding dimension and the GNNs' hidden dimension, since the group-based workload can be shared by multiple threads instead of single thread. 
% % Second, it would facilitate more efficient data access, such as memory coalescing, to improve memory performance. 
% Second, it introduces another performance-related parameter -- the number of working threads along the data dimension for configurability. 


% Besides, we also spot the memory access pattern as a key factor to bring even better performance, since threads with continuous IDs will access to a consecutive part of memory, thus facilitating the memory coalescing on GPUs. To this end, as shown in Figure~\ref{fig: Dimension-based Workload Sharing.}\subfig{b}, we adjust the threads and their workload mapping, where adjacent threads would operate on the dimension close to each other side by side.

% \section{Group-size Selection}
% \todo{simple heuristic to determine the determine the group size }

==> 05_new_GPU_memory_hierarchy.tex <==
\section{Memory Optimization} 
\label{sect: Memory Optimization}
In this section, we detail the memory optimization used in our kernel \& runtime crafter, including \textit{node renumbering} and \textit{memory organization}.

\subsection{Community-aware Node Renumbering} \label{sect: Node Renumbering}
Node renumbering is a way to ``rename'' each node (ID) of a graph to improve the temporal and spatial locality at the GNN aggregation phase. It is based on the idea that the closeness of node IDs would affect the adjacency of the time (\textbf{WHEN} they get processed) and the proximity of the location (\textbf{WHERE} they get handled), such as blocks and SMs in GPU.

Specifically, there are two steps in applying the node renumbering. First, to identify the communities, we leverage Rabbit Clustering~\cite{rabbit-order}, which essentially maximizes the graph modularity by clustering the nodes of graph. Our initial studies also shows that Rabbit Clustering outperforms some other graph clustering/partitioning approaches (\textit{e.g.}, METIS~\cite{METIS} and learning-based partitioning~\cite{sysMLROC}), in terms of better flexibility and lower runtime cost. This step will assign each node with a community index, namely $com\_idx$. Second, we simply assign the nodes within the same community with a intra-community index, namely $local\_idx$, based on the ascending order of their node IDs. After the above two steps, we can get the one-to-one mapping from the old node ID to the new IDs (computed by $com\_idx$ and $local\_idx$). Note that the above renumbering process is lightweight in its computation and memory cost, and can be effectively parallelized~\cite{rabbit-order}. After being processed, nodes within each community would be assigned with IDs continuous in its number values, and nodes with consecutive IDs sharing more neighbors are more likely to be processed with better temporal and spatial locality. We quantify such benefit in Section~\ref{sect: Node Renumbering Benefits}.
% \vspace{-10pt}

\subsection{Block-aware Memory Customization} 
\label{sect: Block-based Workload Mapping}
To exploit the performance benefits from GPU memory hierarchy, \Mname~incorporates an efficient block-aware memory customization to support our 2D Neighbor-Dimension workloads.
% As shown in Figure~\ref{fig: Group-based Workload Mapping}, the workload of node $1$ can be handled by thread $a$, $b$, $c$ based on its group-based workload partitioning. In addition, threads within each GPU block (usually consists of up to 1024 threads) can support multiple nodes for neighbor aggregation simultaneously. In the meantime, each block on GPUs owns the shared memory that can be used to cache the ``hot-spot'' data temporarily for fast memory access from all threads of a block. Similar to the leader-node pattern at intra-group aggregation, we use a leader thread (notate as thread $a$ for node $1$ in Figure~\ref{fig: Group-based Workload Mapping}) of each node to manage the final result updates from the shared memory to the global memory, which can further reduce the overhead of the expensive thread-level synchronization at the global memory. Meanwhile, this strategy also reduces the number of threads that are concurrently working on the memory, alleviating the contention among threads. 
% \begin{figure} [h] \small
%     \centering
%     \includegraphics[width=\columnwidth]{imgs/gpu-workload-mapping.pdf}
%     % \vspace{-20pt}
%     \caption{Group-based Workload Mapping.\todo{add explanation for leader node, add GPU-block}}
%     % \vspace{-13pt}
%     \label{fig: Group-based Workload Mapping}
% \end{figure}
% \vspace{-5pt}
% \subsection{Block-aware Memory Organizing}
% \label{sect: Block-aware Memory Organizing}
% To exploit the shared memory benefits, we tailor the GPU memory organization to support the block-based mapping (Section~\ref{sect: Block-based Workload Mapping}) for 2D neighbor-dimensioni workloads. As shown in Figure~\ref{fig: Group-based Workload Mapping}, each block can handle the aggregation workloads from several nodes. 
Specifically, \Mname~utilizes the fast shared memory to hold the block-level aggregation results by further reducing unnecessary access to global memory. Before the GNN kernel execution, we select leader threads for managing results output. After each block completes all of its execution, the selected leaders threads will flush the shared memory result to the global memory for different workload units of the same node.
% \vspace{-8pt}
\begin{algorithm}[h] \small
    \caption{Block-aware Memory Customization.}
    \label{alg: Memory Organization.}
    \SetAlgoLined
    $num\_units = graph.num\_workload\_unit$\;
    $cnt = 0$; \ $local\_cnt = 0$; \ $last = 0$\;
    \While{$cnt < num\_units$}{
        \If{$cnt \ \% \ thread\_per\_block == 0$}{
            $grpPtr[cnt].node\_shared\_addr = local\_cnt$\;
            $last = grpPtr[cnt].node$\;
            $grpPtr[cnt].unit\_leader = true$\;
        }
        \Else{
            \If {$grpPtr[cnt].node == last$)}{
                $grpPtr[cnt].node\_shared\_addr = local\_cnt$\;
            }
            \Else{
                $local\_cnt++$\;
                $grpPtr[cnt].node\_shared\_addr = local\_cnt$\;
                $last = grpPtr[cnt].node$\;
                $grpPtr[cnt].unit\_leader = true$
            }
        }
        $cnt++$\;
        \If {cnt \% thread\_per\_block == 0}{
            $local\_cnt = 0$\;
        }
    }
\end{algorithm}
% \vspace{-10pt}

As described in Algorithm~\ref{alg: Memory Organization.}, each GPU thread handling one workload unit will have three properties, $node\_shared\_addr$ (the shared memory address that holds the intra-group neighbor aggregation result of a node), $node$ (the global index of the node that the neighbor group belongs to), and $unit\_leader$ (boolean flag indicating whether this thread is responsible for flushing the results to global memory for a node). Note that the value of $thread\_per\_block$ should be determined based on the shared memory size of each block and the embedding size of each node. Algorithm~\ref{alg: Memory Organization.} ($line \ 3 - 24$) shows the major organizing routine that captures several cases. First, if the current thread is the first thread of a block ($line \ 4 - 8$), we select the current thread as the leader thread and allocate shared memory for its aggregation target node. Second, if the current thread is in the middle of a block, we may either 1) keep its target node address in shared memory the same as its predecessor if both of them aggregate towards the same target node ($line \ 10 - 12$), or 2) allocate new shared memory for its target node if they aggregate towards different target nodes ($line \ 13 - 18$).

% Considering the memory and computation resource constraints of a block, as well as the input-level information (\textit{e.g.}, the number of nodes and edges), the number of threads per block should be determined to balance the thread efficiency (\textit{e.g.}, thread management, and resource sharing) at the intra-block level and parallelization at the inter-block level, \todo{where each box represent the node embedding values.} 

% \section{Memory-aware Scheduling}
% \label{sect: Memory-aware Scheduling}
% Besides the aforementioned group-based workload management and memory optimizations, \Mname~leverages efficient memory-aware scheduling to maximize their performance benefits in a hardware friendly manner. It enforces a thread schedule that can capitalize on the neighbor sharing benefits among threads within each GPU-block. We generate the overall thread schedule by interleaving the workloads from different nodes. We describe its process in Algorithm~\ref{alg: Schedule Generation.} based on an initial workload queue, where each element is $(nodeID, \#Group)$. At each iteration ($line \ 5-13$), we generate a  schedule for each thread by popping out workload queue and pushing element ($(threadId, nodeID, GroupID)$) to a schedule list.
% \begin{algorithm}[h] \small
%     \SetAlgoLined
%     $WS$ = \{$(0, wload_0), (1, wload_1), ~\dots, (n, wload_n)$\}\;
%     $id\_counter = 0$ \;
%     $Schedule = \{\}$\;
    
%     \While{$WS.size() > 0$}{
%         $item = WS.pop()$ \;
%         $nid  = item[0]$ \; 
%         $gid  = item[1] - 1$ \;
%         $Schedule.push((id\_counter, nid, gid))$\;
%         \If{$gid > 0$}{
%             $new\_item = (nid, item[1] - 1)$\;
%             $WS.push(new\_item)$\;
%         }
%         $id\_counter++$\;
%     }
% \caption{Schedule Generation.}
% \label{alg: Schedule Generation.}
% \end{algorithm}

% \vspace{-10pt}
% After applying the above algorithm, the actual schedule of the groups can be illustrated in Figure~\ref{fig: Memory-aware Scheduling.}. It can be seen that the groups from consecutive nodes are placed continuously (\textit{e.g.}, group $c$ from node $1$ and node $3$ are placed side by side) while groups from the same node are interleaved (\textit{e.g.}, group $a$ and group $b$ from node $1$ are placed away from each other). The major insight behind this strategy is that the node renumbering will maximize the neighbor sharing among nodes with consecutive IDs, therefore, we prioritize placing the groups from nodes with adjacent IDs close enough to each other to improve the spatial and temporal locality during node aggregation.
% \begin{figure} [h] \small
%     \centering
%     \includegraphics[width=\columnwidth]{imgs/group-based-scheduling.pdf}
%     \caption{Memory-aware Scheduling.}
%     \vspace{-15pt}
%     \label{fig: Memory-aware Scheduling.}
% \end{figure}


==> 06_Profiling_and_Modeling.tex <==
% \section{Modeling, Profiling and Estimating} \label{sect: Modeling, Profiling and Estimating}
% \vspace{-10pt}
\section{Design Optimization}
% \vspace{-5pt}
\label{sect: Performance Evaluator}
In this section, we introduce the design optimization through the performance evaluator of \Mname, which includes the \textit{Modeling} and \textit{Estimating}. As illustrated in Figure~\ref{fig: Overall optimization flow}, the performance evaluator takes the input settings (Graph, GNN, and GPU parameters)) that are captured by our input extractor, to determine the optimizations that will be executed by kernel \& runtime crafter.
\begin{figure} [h] \small
    \centering
    \includegraphics[width=\columnwidth]{imgs/optimization-flow.pdf}
    % \vspace{-25pt}
    \caption{Overall Optimization Flow.}
    % \vspace{-10pt}
    \label{fig: Overall optimization flow}
\end{figure}

% \vspace{-5pt}
\subsection{Modeling}
% \vspace{-5pt}
\label{sect: Modeling}
Modeling basically measures the performance impact of hyper-parameters of system-level optimizations. Three major hyper-parameters have been utilized.
% \subsubsection{Community Size} \label{sect: community size}
% Graph community size ($csize$) determines the granularity at which we could ``partitioning the graph'' and how we could handle each community efficiently. This factor has relation with the locality performance and efficiency, such as a large community can have the opportunity to share more neighbors. However, in the meantime, it would become more challenging to capitalize such benefits on GPU, which is usually limited by the compute capability and memory resources. Our analytical modeling for the relation between $\#community$ and latency can be formulated as
% \begin{equation}\small \label{equ: latency vs community size}
%     Latency_{csize} = \frac{\#E}{csize} \times (1 + |csize - \sqrt{\frac{\#N}{\#E}}\frac{\#N}{\epsilon}|).
% \end{equation}
% where the input-level information has been used, such as $\#N$ (the number of nodes) and $\#E$ (the number of edges). $\epsilon$ is a hyper-parameter and its value is based on the ideal number of nodes of each community that can fit into the L2 cache of GPU.
% \subsubsection{Group Size} \label{sect: group size}

\vspace{2pt}
\textbf{Group Size ($gs$):} $gs$ balances the workloads and reduces the overhead of the inter-thread synchronization (\textit{e.g.}, atomic operations). The increase of the $gs$ will reduce the frequency of thread synchronization and memory access. However, when $gs$ becomes even larger than most of the node degrees, such benefit will diminish due to the irregular size of each unfulfilled group. Increasing $gs$ also requires more work on a single thread while compromising parallelization. On the other side, if we aggressively decrease $gs$, it may underutilize each thread, since it cannot fulfill the computation capability of each thread to offset thread launching cost.

\vspace{2pt}
\textbf{Thread-per-block ($tpb$):} $tpb$ balances the intra-block and inter-block efficiency. First, the increase of $tpb$ will accommodate more groups in each thread block. Meanwhile, the inter-thread contention in each block will become severer. On the contrary, if we decrease the $tpb$ too much, the temporal and spatial locality of neighbor sharing would diminish. Besides, $tpb$ would also affect the total number of blocks that will be running in parallel, which impacts the resource isolation and scheduling flexibility.

\vspace{2pt}
\textbf{Dimension Worker ($dw$):} $dw$ partitions the aggregation workloads along the node embedding dimension and distributes them to multiple threads. The increase of $dw$ would benefit the computation parallelization, which contributes to the overhead performance in terms of reduced latency. Meanwhile, the value of $dw$ should also make a tradeoff between the single-thread efficiency and multi-thread parallelization.

To estimate the runtime latency, we use the formula,
\begin{equation} \small \label{equ: latency and group size}
Latency = \frac{E\times D}{gs\times |dw - {D}/3| \times |tpb - \sqrt{max\_tpb}|} \times (1 + |gs - \alpha\frac{N}{E}|).
\end{equation}
where $N$ is the number of the nodes; $E$ is the number of edges; $max\_tpb$ is the maximum number thread a block can hold; $D$ is the node embedding dimension; $\alpha$ is to handle different graphs with node degree variations (based on the standard deviation of node degree ($stddev_{degree}$)). Our insight is that if the value of $gs$ can approach $\alpha\frac{N}{E}$ either from its left side (lower) or right side (higher), the performance will become better. The larger $stddev_{degree}$ is, the higher the value of $\alpha$ becomes. We set $\alpha$ in the range of $0.15$ to $0.3$. 

In addition, we should respect the single-thread efficiency
\begin{equation} \small
    0 < \frac{gs \times D}{dw} \leq computation\_capability.
\end{equation}
where $computation\_capability$ of each thread can be measured by computation throughput (GB/s) of SMs on GPUs. Meanwhile, we should consider the shared memory size ($memory\_capacity$) of each block,
\begin{equation} \small
    0 < \frac{tpb\times gs}{avg\_degree\times dw} D \times bytes_{type} \leq memory\_capacity.
\end{equation}
where $avg\_degree$ is the average degree of each node; $bytes_{type}$ is the size of data type (4 bytes for floating point).
% \vspace{-5pt}
% \subsubsection{Thread per Block}
% \vspace{-5pt}
% \label{sect: thread per block}
% Thread-per-block is another major factor to balance intra-block and inter-block efficiency. It impacts the performance from two perspectives. First, the increase of thread-per-block will lead to accommodate more groups in each thread block. Meanwhile, the inter-thread contentions in each block will become severe. On the contrary, if we decrease the threads-per-block, the temporal and spatial locality of neighbor sharing would diminish. Second, thread-per-block would also affect the total number of blocks that will be running in parallel, which would gain additional benefit of resource (memory) isolation and scheduling flexibility. We also provide an analytical model to measure thread-per-block (TPB) impact on latency and resources:
% \begin{equation} \small \label{equ: latency vs TPB}
%     Latency_{TPB} = \frac{E}{TPB}\times (1 + |TPB - \theta \frac{M\sqrt{\frac{N}{E}}}{D\times bytes_{type}}|).
% \end{equation}
% where $M$ is the shared memory size for each block of threads. $TPB$ is also constrained by compute and memory constraints of each block:
% \begin{equation} \small
%     0 < TPB \leq max\_num\_thread\_per\_block.
% \end{equation}
% where $max\_num\_thread\_per\_block$ is usually a hardware limit (1024 for CUDA), and
% \begin{equation} \small
%     0 < \sigma \times TPB \times D \times bytes_{type} \leq block\_mem.
% \end{equation}
% where $block\_mem$ is the size of shared memory, and $\sigma$ is a metric to measure the overlapping of nodes in each block, which can be computed by neighbor sampling and set-intersection operation.

% \vspace{-10pt}
\subsection{Estimating} \label{sect: profiling and estimating}
While the graph structure would vary from the graph to graph, their underlying community structures are relatively fixed in sizes and shapes. Based on this observation, we propose a community-based GNN profiling strategy, which could largely ease the profiling efforts. Specifically, we follow three major steps. First, we broadly collect the most typical sizes of the graph community, and randomly generate the edge connections with 90\%, 70\%, and 50\% densities. Second, we evaluate them on \Mname~based on the several most popular sizes (\textit{e.g.}, 16 in GCN, 256 in GIN) of the GNN hidden layer embedding size, group size, and thread-per-block size. Note that this step will also help us to explore the best value of hyper-parameters $\alpha$ (Equation~\ref{equ: latency and group size}) under different settings. Third, we select a set of appropriate hyper-parameters to approximate the overall performance for a given input setting. To this end, we can easily get a ``sense'' of how good or bad for a given GNN input.

To optimize hyper-parameters, we 1) start from a set of randomly generated settings based on previous profiling results; 2) approximate their performance based on the above method and keep the settings that can deliver high enough performance; 3) do crossover on these kept settings to generate a new set of settings for the next iteration beginning from step 2. In general, 10 - 15 iterations of the above process would be enough to generate a ``premium'' setting with a satisfying performance that can meet the users' requirements. 

